Nonlinear thermoelectric response of quantum dots: renormalized dual fermions out of equilibrium

The thermoelectric transport properties of nanostructured devices continue to attract attention from theorists and experimentalist alike as the spatial confinement allows for a controlled approach to transport properties of correlated matter. Most of the existing work, however, focuses on thermoelectric transport in the linear regime despite the fact that the nonlinear conductance of correlated quantum dots has been studied in some detail throughout the last decade. Here, we review our recent work on the effect of particle-hole asymmetry on the nonlinear transport properties in the vicinity of the strong coupling limit of Kondo-correlated quantum dots and extend the underlying method, a renormalized superperturbation theory on the Keldysh contour, to the thermal conductance in the nonlinear regime. We determine the charge, energy, and heat current through the nanostructure and study the nonlinear transport coefficients, the entropy production, and the fate of the Wiedemann-Franz law in the non-thermal steady-state. Our approach is based on a renormalized perturbation theory in terms of dual fermions around the particle-hole symmetric strong-coupling limit.

==> PaxHeaders.26617/manuscript_thermo.tex <==
20 atime=1358245276
20 ctime=1358245274

